Follow Your Path: a Progressive Method for Knowledge Distillation

Deep neural networks often have a huge number of parameters, which posts challenges in deployment in application scenarios with limited memory and computation capacity. Knowledge distillation is one approach to derive compact models from bigger ones. However, it has been observed that a converged heavy teacher model is strongly constrained for learning a compact student network and could make the optimization subject to poor local optima. In this paper, we propose ProKT, a new model-agnostic method by projecting the supervision signals of a teacher model into the student's parameter space. Such projection is implemented by decomposing the training objective into local intermediate targets with an approximate mirror descent technique. The proposed method could be less sensitive with the quirks during optimization which could result in a better local optimum. Experiments on both image and text datasets show that our proposed ProKT consistently achieves superior performance compared to other existing knowledge distillation methods.

==> 061experiments_nlp.tex <==
% \subsection{Text Classification}
% In this section, we empirically verify the validity of \method in text classification tasks. 

% \subsubsection{Setup}

% Text classification experiments are conducted following the setting of \cite{turc2019well} and \cite{tinybert}.

% \noindent\textbf{Datasets}.
% We evaluate our method for sentiment classification on SST-2~\cite{sst-2}, natural language inference on MNLI~\cite{mnli} and QNLI~\cite{qnli}, and paraphrase similarity matching on MRPC~\cite{mrpc} and QQP\footnote{ https://data.quora.com/First-Quora-Dataset-Release-Question-Pairs.}.

% \noindent\textbf{Settings}. The teacher model is the  BERT-base \cite{bert} fine-tuned in the training set, which is a 12-layer Transformers~\cite{vaswani2017attention} with  768 hidden units. Following the setting of \cite{turc2019well} and \cite{tinybert}, a BERT of 6 layer Transformers and 786 hidden units is conducted as the student model. We use the pre-trained BERTs released by \cite{turc2019well}.
% In order to evaluate our method in the setting of students with different structures with the teacher, a single-layer bi-LSTM with 300 embedding size and 300 hidden size is used as another student model. We fine-tune 4 epoch for non-distillation training and 6 epoch for distillation training. Adam~\cite{adam} optimizer with learning rate 0.001 is used for biLSTM and with a learning rate from \{3e-5, 5e-5, 1e-4\} is used for BERTs. The hyper-parameter of $\lambda$ in Eq.~\ref{eq:constrain} is chosen according to the performance in the validation set.


% \noindent\textbf{Baselines}. We compare our method with following baselines: (1) BERT + Finetune, fine-tune the BERT student on training set;  (2) BERT/bi-LSTM + KD, fine-tune the BERT student or train the bi-LSTM on training set using the vanilla knowledge distillation loss~\cite{hinton2015distilling}; (3) Route Constrained Optimization (RCO)~\cite{jin2019knowledge}, use 4 un-convergent teacher checkpoints as mediate training target; (4) bi-LSTM: train bi-LSTM in training set. For vanilla KD methods,  we set the temperature as 1.0 and only use the KL divergence with teacher outputs as loss. We also compare our method with the results reported by \cite{sun2019patient} and \cite{turc2019well}.



% \subsubsection{Baselines}

% \begin{itemize}
%     \item PF: without distillation, pre-training + fine-tuning.
%     \item PD: pretraining + vanilla distillation using KL divergence between student and teacher.
%     \item RCO: Route Constrained Optimization. using non-convergent checkpoints of teacher as mediate training target. 
%     \item TinyBERT~\cite{tinybert}. Except the output probability of teacher, using the attention, hidden states and embedding of teacher as other supervision.
% \end{itemize}

\subsubsection{Results and discussion}

The accuracy or f1-score on test set are shown in Tab.~\ref{tab:glue}. All results are obtained by submitting to the GLUE~\cite{wang2018glue} website.  Results show that our method could improve the performance of knowledge distillation in natural language as well. 
Our model is effective for not only smaller BERT student but also student with other architecture, such as RNN. Especially, when the student is bi-LSTM, directly distilling knowledge from a pre-trained BERT has a minor effect. Our model, who learns from the pretraining trajectory of the teacher is much more effective in distilling the knowledge from BERT. Similarly, as shown in Fig.~\ref{fig:lambda_mnli}, the performance is not sensitive to the $\lambda$ when the $\lambda$ is not too large.







